Using Pi-Calculus Names as Locks

Locks are a classic data structure for concurrent programming. We introduce a type system to ensure that names of the asynchronous pi-calculus are used as locks. Our calculus also features a construct to deallocate a lock once we know that it will never be acquired again. Typability guarantees two properties: deadlock-freedom, that is, no acquire operation on a lock waits forever; and leak-freedom, that is, all locks are eventually deallocated. We leverage the simplicity of our typing discipline to study the induced typed behavioural equivalence. After defining barbed equivalence, we introduce a sound labelled bisimulation, which makes it possible to establish equivalence between programs that manipulate and deallocate locks.

==> eptcsdata.tex <==
\providecommand{\firstpage}{76}
\providecommand{\publicationstatus}{G. Caltais and C. A. Mezzina (Eds): Combined Workshop on\\
Expressiveness in Concurrency and Structural Operational Semantics\\(EXPRESS/SOS 2023).\\
EPTCS 387, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.387.7}{10.4204/EPTCS.387.7}}

